Latent Abstractions in Generative Diffusion Models

In this work we study how diffusion-based generative models produce high-dimensional data, such as an image, by implicitly relying on a manifestation of a low-dimensional set of latent abstractions, that guide the generative process. We present a novel theoretical framework that extends NLF, and that offers a unique perspective on SDE-based generative models. The development of our theory relies on a novel formulation of the joint (state and measurement) dynamics, and an information-theoretic measure of the influence of the system state on the measurement process. According to our theory, diffusion models can be cast as a system of SDE, describing a non-linear filter in which the evolution of unobservable latent abstractions steers the dynamics of an observable measurement process (corresponding to the generative pathways). In addition, we present an empirical study to validate our theory and previous empirical results on the emergence of latent abstractions at different stages of the generative process.

==> experiment_new.tex <==
\subsection{Probing}
The probing technique, as described in \cite{alain2016understanding}, involves training linear classifiers on feature maps extracted from different layers of a neural network. This method is employed to investigate the internal representations that the network learns at various stages of processing. In our case, the U-Net NCSPP model comprises 162 layers, including both linear and convolutional layers.

\textbf{Dataset and Model Configuration}

For our experiments we selected two dataset: Shapes3D \cite{kim2018disentangling}, a collection of 64x64 images depicting simple scenes which features varying colored objects such as spheres and cubes with a scale and orientation, positioned against differently colored walls and floors and CELEBAHQ \cite{karras2017progressive} which features 256x256 images focusing on human facial attributes. For our experiments, we utilized the U-Net NCSPP model \cite{song2021a}.

Initially, we trained the U-Net NCSPP model unconditionally, using score-matching objective\cite{song2021a}.
Once the model was successfully trained, we selected a specific subset of the dataset for the probing experimentation. This subset was divided into 246 training examples, 150 validation examples, and 371 test examples. To ensure fairness and rigor in model evaluation, we employed a multilabel stratification algorithm \cite{sechidis2011stratification} \cite{pmlr-v74-szymański17a}, guaranteeing a balanced distribution of labels across all dataset splits.
Each image in this subset was then subjected to noise corruption using a variance-exploding noise schedule \cite{song2021a}, with noise levels increasing from 0 to 1 in steps of 0.1. This process resulted in a series of progressively corrupted images at each noise level, as depicted in Figure \ref{fig:noise}. These images served as inputs to the model from which we extract the feature maps from all the linear and convolutional layers of the model.
For each level of noise corruption, we extracted feature maps from every layer of the model, resulting in a total of 162 feature map sets for each noise level. This process yielded 11 (from 0 to 1 noise levels in steps of 0.1) different datasets per layer, each corresponding to a different noise condition.
We then trained a linear classifier for each of these datasets using the training subset. Classifier performance was optimized by selecting models based on their log-probability accuracy observed on the validation subset. The final evaluation of each classifier was conducted on the test subset.

\textbf{Internal Representation and Feature Maps}

Our findings corroborate empirical observations from related studies \cite{chen2023beyond}, indicating that certain general features like wall hue and floor hue in Shapes3D, and attributes like gender and age in CELEBA are determined early in the diffusion process (noise levels around 0.1 to 0.2), while more specific features such as object hue, shape, scale, and orientation for Shapes3D and bangs, eyeglasses for CELEBA emerge at later stages (noise levels around 0.3 to 0.4) suggesting that the model commits to certain decisions regarding these features later on.
Figure \ref{fig:probing} compares the efficacy of linear probes applied to the model's internal feature maps against those applied directly to the noisy images. The raw, corrupted images consistently yielded lower classification accuracy, underlining the inability of a linear classifier to effectively decipher labels from such data. Conversely, the accuracy significantly improved in intermediate layers, affirming that the model constructs a robust internal representation of the image attributes.


\subsection{Mutual Information Analysis} 
Mutual Information (MI) is a metric for quantifying the non-linear dependencies between random variables. In the context of our study, we aim to assess the MI between the labels and the outputs of the diffusion model across varying diffusion times. This analysis is intended to reveal how the model's internal representations evolve and how they relate to the observable outputs at different stages of the diffusion process.

\textbf{Eperimental Setup}

 We adopted the MINDE-C technique from \cite{franzese2024minde} to compute the MI. This involved training conditional diffusion models on the entire Shapes3D dataset with a mixed conditioning scheme: 33\% of training instances were conditioned on all labels, 33\% on a single label, and the remaining 33\% were trained unconditionally. 


For the MI estimation, we employed the same test set split (371 test examples) used in the previous probing experiments.
Using the MINDE-C algorithm, we leveraged score-functions to compute the Kullback-Leibler divergence between the conditional and marginal distributions of the model's outputs. This computation provided a quantitative measure of the MI for each label.

\textbf{Bridging the Gap Between Empirical Probing and Theoretical Insights}

Figure \ref{fig:mi} presents a comparative analysis of the mutual information dynamics and the probing results over time. The patterns observed across both measures are similar, reinforcing our hypothesis about the link between observable and latent worlds. Mutual information estimate can serve as a theoretical and empirical tool to study information flow in generative models and  how information about various attributes is encoded and preserved throughout the diffusion process.



\begin{figure}[ht]
    \centering
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/features_vs_pixel_new.png}
        \caption{Feature map vs Noisy image}
        \label{fig:probing}
    \end{minipage}\hfill
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/mi_vs_features_new.png}
        \caption{Mi vs features map}
        \label{fig:mi}
    \end{minipage}
\end{figure}


\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]{figures/noisy_balls.png}
    \caption{Noise over time}
    \label{fig:noise}
\end{figure}

\begin{figure}[ht]
    \centering
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/features_vs_pixel.png}
        \caption{Placeholder}
        \label{fig:probing}
    \end{minipage}\hfill
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/mi_vs_features.png}
        \caption{Placeholder}
        \label{fig:mi}
    \end{minipage}
\end{figure}


\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]{figures/noisy_balls.png}
    \caption{Placeholder}
    \label{fig:noise}
\end{figure}


==> linear_diffusion.tex <==

Although the discussion in this work includes a large class of measurement function, we here is to specialize the framework to the particular case of linear generative diffusion models \cite{song2021a}. Typically, these models are presented through the lenses of time reversal of \glspl{SDE} \cite{anderson1982reverse}. The simple connection between this formalism and the one considered in this paper is explored in the following.

Consider on $\ccU$ the \textit{reversed} process $\hat{Y}_t\defeq Y_{T-t}$ and the associated filtration $\cF_t^{\hat{Y}}\defeq\sigma(\hat{Y}_{0\leq s\leq t}) = \sigma(Y_{T-t\leq s\leq T})$. The measure $\PO$ is selected such that the process $\hat{Y}_t$ has ($\cF_t^{\hat{Y}}$ adapted) expression
\begin{equation}\label{eq:diffmod}
\hat{Y}_t=\hat{Y}_0-\alpha \int\limits_{0}^t \hat{Y}_{s}\dd s+\hat{W}_t,%=\exp(-\alpha t)\hat{Y}_0+\hat{W}_t,
%\rightarrow Y_{T-t}=Y_T+\alpha \int\limits_{T-t}^{T} Y_{s}\dd s+\hat{W}_t
\end{equation}
where we consider a Brownian motion $\{\hat{W}_t,\cF_t^{\hat{Y}}\}$,
for a given $\alpha\geq 0$. Particular choices of $\alpha$ corresponds to the so called Variance-Preserving and Variance Exploding schedules of diffusion models \cite{song2021a}. In this exposition we consider \Cref{assumption1} valid, which implies that we should select $\hat{Y}_0=Y_T=\rX$. In diffusion models jargon, \Cref{eq:diffmod} is typically referred to as a \textit{noising} process. The reason for such a name can be understood by analysing the evolution of \Cref{eq:diffmod} where $\hat{Y}_{t}$ became a noisier and noisier version of $\rX$ as $t$ grows ( in particular, $\hat{Y}_t=\exp(-\alpha t)\rX+\exp(-\alpha t)\int_0^t \exp(\alpha s)\dd \hat{W}_s$). Clearly \Cref{eq:diffmod} is equivalent to $Y_{t}=Y_T-\alpha \int\limits_{t}^{T} Y_{s}\dd s+\hat{W}_{T-t}$ which is an expression for the original $Y_t$ process which is adapted to $\cF^{\hat{Y}}$. Our goal is as follows: first, we derive an expression for $Y_t$ which is $\cF^{Y,X}_t$ adapted and in the form of \Cref{eq:param_sde}. Then, we derive the version which is $\cF^Y_t$ adapted, and finally show that such a process coincides with the generative dynamics of linear diffusion models.

We select for the moment $\alpha=0$ for simplicity, although our discussion will be easily extended. The process $Y_t$ can be expressed in this case as $Y_t=Y_T+\hat{W}_{T-t}=Y_0+Y_T-Y_0+\hat{W}_{T-t}$. Since the process $\hat{W}_t$ is $\sigma(\hat{Y}_0,\hat{Y}_t)$ adapted, equivalently $\sigma(Y_T,Y_{T-t})=\sigma(\rX,Y_{T-t})$, we recognize that $Y_t$ can be written as $Y_0$ plus the process $Y_T-Y_0+\hat{W}_{T-t}$ which is $\sigma(\rX,Y_{t},Y_{0})$ adapted. Since $\sigma(\rX,Y_{t},Y_{0})\subset \cF^{Y,X}_t$, such process is also adapted to the bigger filtration. We consider then the process $\frac{\rX-Y_t}{T-t}$ and through some trivial algebraic manipulation write
\begin{equation}\label{eq:genparam_ve}
    Y_t=Y_0+\int_0^t\frac{\rX-Y_s}{T-s}\dd s+\underbrace{\left(Y_T-Y_0+\hat{W}_{T-t}-\int_0^t\frac{\rX-Y_s}{T-s}\dd s\right)}_{M_t}.
\end{equation}
The important claim is then the following: $\{M_{0\leq t\leq T},\cF^{Y,X}_{0\leq t\leq T}\}$ is a Brownian motion (\hyperref[proof:mt_brownian]{[Proof]}\label{hyper_label}). Then, \Cref{eq:genparam_ve} is in the form of \Cref{eq:param_sde} and casting \Cref{eq:system} for the particular case of interest we can obtain generative dynamics. 

%\begin{flalign*}
%    &Y_{t}=Y_0+\alpha \int\limits_{0}^{t} Y_{s}\dd s+Y_T-Y_0-\alpha \int\limits_{0}^{t} Y_{s}\dd s+\alpha \int\limits_{t}^{T} Y_{s}\dd s+\hat{W}_{T-t}
%\end{flalign*}
Actually, generative dynamics can be obtained following a different path: finding starting from the process which is $\cF^{\hat{Y}}$ adapted, the time reversal of such dynamics.
The fundamental result borrowed from \cite{anderson1982reverse} in \cite{song2021a} is the fact that the time reversal of a diffusion process is (provided technical conditions) again a diffusion process, where the drift term contains an extra term called \textit{score-function}. Consequently, it is possible to write $Y_t$ in a form that is adapted w.r.t. $\cF^Y$, and thus amenable to simulation for generative modelling purposes. The key element in the derivation of \cite{anderson1982reverse} is the score function $s(y,t)$, defined as the gradient of the logarithm of the Radon-Nikodym derivative of the instantaneous measure $\PO(Y_t\in \dd y)$ w.r.t. the Lebesgue measure in $\mathbb{R}^N$. In practical terms, $s(y,t)=\nabla\log \rho(y,t)$, where $\PO(Y_t\in \dd y)=\rho(y,t)\dd y$. Notice that this score should exist. For this reason, similarly to what discussed previously, the analysis of the existence of the process adapted to $\cF^Y_t$ is considered in the time interval $[0,T)$ \citep{haussman2}. Depending on the considered scenario, again this restriction can be relaxed, but for simplicity we avoid this discussion here.


Whenever the diffusion process is selected in the form of \Cref{eq:diffmod}, the score function has a particularly simple known form. We restate hereafter the content of \cite{anderson1982reverse, song2021a} by adopting our notation
\begin{theorem}\label{anders_thm}
    Consider the stochastic process $Y_t$ which solves \Cref{eq:diffmod}. The same stochastic process also admits $\cF^Y_t$ adapted representation
    \begin{equation}\label{eq:songsde}
        Y_t=Y_0+\int_0^t \alpha Y_s+\underbrace{2\alpha\frac{\exp(-\alpha (T-s))\E_{\PO}[\rX\g \sigma(Y_s)]-Y_s}{1-\exp(-2\alpha (T-s))}}_{\text{score-function}} \dd s  +W_t,
    \end{equation}
    where $Y_0=\exp(-\alpha T)\rX+\sqrt{\frac{1-\exp(-2\alpha T)}{2\alpha}}\epsilon$, with $\epsilon$ a standard Gaussian random variable independent of $\rX$ and $W_t$.
\end{theorem}
We stress for the interested reader that the same conclusion of \Cref{anders_thm} can be be obtained leveraging the results in \cite{pardoux2006grossissement} (Thm 2.2) by considering \textit{enlargement} of filtrations. The technical connection between time reversal of \glspl{SDE} and the version of a process adapted to an enlarged filtration is explored in \cite{al1987enlarged}, in particular Thm. 3.3 where it is proved how $\beta_t$ of \Cref{bridge} is a Brownian motion.

%Such result, which holds for generic nonlinear diffusion 

What we show here is that the same generative dynamics can be obtained under the nonlinear filtering formalism, without the explicit need of defining a backward and a forward process. In particular, we can directly select a measurement function that corresponds to an Orstein-Uhlenbeck bridge \citep{mazzolo2017constraint,corlay2013properties}, consequently satisfying  \Cref{assumption1}, and obtain the generative dynamics of the classical diffusion models. These dynamics can be considered as a particular case of \Cref{bridge}, when selecting a \textit{linear} function $F$. In particular we consider the following about $H$
\begin{assumption}\label{assumption2}
   The function $H$ is selected to be of the \textit{linear} form 
  % \begin{equation}
  %     H(Y_t,X,t)=-\alpha X+\frac{2\alpha \exp(-\alpha (T-t))}{1-\exp(-2\alpha (T-t))} (X-\exp(-\alpha (T-t))Y_t)
  % \end{equation}
   \begin{equation}
       H(Y_t,X,t)=m_t \rX- \frac{\dd \log m_t}{\dd t} Y_t
   \end{equation}


with $m_t=\frac{\alpha}{\sinh{(\alpha(T-t))}}$, where $\alpha\geq 0$. When $\alpha=0$, $m_t=\frac{\dd \log m_t}{\dd t}=\frac{1}{T-t}$. Furthermore, $Y_0$ is selected as in \Cref{anders_thm}. 

\end{assumption}
Under this assumption, $Y_T=\rX,\quad \PO-a.s.$, as can easily be checked thanks to the following equality \hyperref[proof_eq:analydiff]{[Proof]}\begin{equation}\label{eq:analydiff}
    Y_t=Y_0\frac{m_0}{m_t}+\rX\frac{m_0}{m_{T-t}}+\int_0^t \frac{m_{s}}{m_t}\dd W_s.
\end{equation} 
When combining \Cref{innovation_theo} with \Cref{assumption1} we obtain that  the process $Y_t$ is equal to 
\begin{equation}\label{gen_sde}
    Y_t=Y_0+\int_0^t m_s \E_{\PO}(\rX\g \cF^{Y}_s)\dd s-\int_0^t \frac{\dd \log m_s}{\dd s} Y_s\dd s+{W}^{\cF^Y}_t,
\end{equation}
which is nothing but \Cref{eq:songsde} after some simple algebraic manipulation. The only relevant detail worth deeper exposition is the clarification about the actual computation of expectation of interest. If $\PO$ is selected such that $\hat{Y}_t$ solves \Cref{eq:diffmod}, we have that 
\begin{equation}
    \E_{\PO}(\rX\g \cF^{Y}_t )=\E_{\PO}( Y_T \g \sigma(Y_{0\leq s\leq t}) )=\E_{\PO}( \hat{Y}_0 \g \sigma(\hat{Y}_{T-t\leq s\leq T}))=\E_{\PO}( \hat{Y}_0 \g \sigma(\hat{Y}_{T-t}))=\E_{\PO}( \rX \g \sigma(Y_t)),
\end{equation}
where the second to last equality is due to the Markov nature of $\hat{Y}_t$.

%In a similar fashion to what done in the previous subsection, we can explicitely write generative diffusion models as \textit{systems} of \glspl{SDE} 
%\begin{equation}\label{eq:systemlin}
%    \boxed{\color{red}\begin{cases}
%        \langle\piphit,\rX\rangle=\langle \piphiz, \rX\rangle+\int\limits_0^t m_s\left(\langle \piphis, \rX^2\rangle-\langle \piphis, \rX\rangle^2\right) \left(\dd Y_s-(m_s\langle \piphis, \rX\rangle-\frac{\dd\log m_s}{\dd s}Y_s)\dd s
%\right)\\
%Y_t=Y_0+\int_0^t \left(m_s\langle \piphis, \rX\rangle -\frac{\dd\log m_s}{\dd s}Y_s \right) \dd s+{W}^{\cF^Y}_t.    
%\end{cases}}
%\end{equation}   
Moreover, in this particular case we can express the mutual information $\cI(Y_{0\leq s\leq t};\gX)=\cI(Y_{t};\gX)$ ( where we removed the past of $Y$ since the following Markov chain holds $\gX\rightarrow \hat{Y}_0\rightarrow \hat{Y}_{t>0}$) can be expressed in the simpler form
\begin{equation}\label{MI_eq_diff}
      \cI(Y_{t};\gX)= \cI(Y_{0};\gX)+ \frac{1}{2}\E_{\PO}\left[ \int_0^t m^2_s\norm{\E_{\PO}[\rX \g \sigma(Y_s)]-\E_{\PO}[\rX \g \sigma(Y_s, \gX)]}^2 \dd s \right]
\end{equation}

\begin{comment}
\Cref{minde:eq_diff} allows to investigate how to compute the mutual information between $\gX$ and the random variable (for a fixed $t$) $\E_{\PO}[\rX \g \sigma(Y_t)]$. We overload the notation of \Cref{sec:NLF} and define a new $\cS^{\dagger}$ as $\cS^{\dagger}= \cS \times \mathbb{R}^N$. The new latent abstraction is obtained as $X^{\dagger}= [X,\E_{\PO}[\rX \g \sigma(Y_t)]]$, and the new "\textit{rendering}" variable as $V^{\dagger}= \E_{\PO}[\rX \g \sigma(Y_t)]$.
Then we can re-use all the derived equations to claim that
\begin{equation}\label{minde:eq_exit}
          \cI(\E_{\PO}[\rX \g \sigma(Y_t)];\gX)= \cI(Y_{0};\gX)+ \frac{1}{2}\E_{\PO}\left[ \int_0^T m^2_s\norm{\E_{\PO}[\rX^\dagger \g \sigma(Y_s)]-\E_{\PO}[\rX^\dagger \g \sigma(Y_s, \gX)]}^2 \dd s \right]
\end{equation}



\end{comment}

















==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> model_figure.tex <==

\begin{figure}[h]
\centering
\begin{subfigure}{.5\textwidth}
\begin{tikzpicture}[node distance=1cm, auto]

% Nodes
\node (X) [draw, rectangle, rounded corners] {$X$};
\node (Y) [right of=X, draw, rectangle, rounded corners] {$Y_t$};
\node (phi) [below of=Y, draw, rectangle, rounded corners] {$\piphit$};

% Arrows
\draw[->, color=red] (X) -- (Y);
\draw[->] (Y) -- (phi);
\draw[->] (Y) edge[loop above] (Y);
\draw[->] (phi) edge[loop below] (phi);

% Labels
%\node [below of=X, node distance=1cm] {Latent \\Abstraction};
%\node [below of=Y, node distance=1cm] {Measurement Process};
\node [right of=phi, node distance=4cm] {$\dd\pi_t= \pi_t\left(H-\langle \piphit,H\rangle\right) \left(\dd Y_t-\langle \piphis,H\rangle\dd t\right)$};
\node [right of=Y, node distance=3cm] {$\dd Y_t= H(Y_t,{\color{red}X},t)\dd t+\dd W_t$};

\end{tikzpicture}
\caption{Nonlinear Filtering: Interaction between Latent Abstraction $X$, Measurements $Y_t$, and Filtering process $\piphit$}
\label{fig:interaction}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
\begin{tikzpicture}[node distance=1cm, auto]

% Nodes
\node (X) [draw, rectangle, rounded corners] {$X$};
\node (Y) [right of=X, draw, rectangle, rounded corners] {$Y_t$};
\node (phi) [below of=Y, draw, rectangle, rounded corners] {$\piphit$};

% Arrows
\draw[->] (X) edge[dashed] (Y);
\draw[->] (Y) -- (phi);
\draw[->] (Y) edge[loop above] (Y);
\draw[->] (phi) edge[loop below] (phi);
\draw[->] (phi) edge[bend left, color=red] (Y);
\draw[->] (phi) edge[dashed] (X);

% Labels
%\node [below of=X, node distance=1cm] {Latent \\Abstraction};
%\node [below of=Y, node distance=1cm] {Measurement Process};
\node [right of=phi, node distance=4cm] {$\dd\pi_t= \pi_t\left(H-\langle \piphit,H\rangle\right) \left(\dd Y_t-\langle \piphis,H\rangle\dd t\right)$};
\node [right of=Y, node distance=3cm] {$\dd Y_t= {\color{red}\langle\piphit,H\rangle}\dd t+\dd W^{\cF^Y}_t$};
\end{tikzpicture}
\caption{Simulated Nonlinear Filtering: Interaction between Measurements $Y_t$, and Filtering process $\piphit$. Latent abstractions updates are \textit{implicitly} simulated (dashed line)}
\label{fig:interaction}
\end{subfigure}
\end{figure}


==> model_figure_simple.tex <==

\begin{figure}[h]
\centering
\begin{subfigure}{.48\textwidth}
\begin{tikzpicture}[node distance=1cm, auto]

% Nodes
\node (X) [draw, rectangle, rounded corners] {$X$};
\node (Y) [right of=X, draw, rectangle, rounded corners] {$Y_t$};
\node (phi) [below of=Y, draw, rectangle, rounded corners] {$\piphit$};

% Arrows
\draw[->, color=red] (X) -- (Y);
\draw[->] (Y) -- (phi);
\draw[->] (Y) edge[loop above] (Y);
\draw[->] (phi) edge[loop below] (phi);

% Labels
%\node [below of=X, node distance=1cm] {Latent \\Abstraction};
%\node [below of=Y, node distance=1cm] {Measurement Process};

\end{tikzpicture}
\caption{Interaction between Latent Abstraction $X$, Measurements $Y_t$, and Filtering process $\piphit$}
\label{fig:interaction}
\end{subfigure}
\begin{subfigure}{.48\textwidth}
\begin{tikzpicture}[node distance=1cm, auto]

% Nodes
\node (X) [draw, rectangle, rounded corners] {$X$};
\node (Y) [right of=X, draw, rectangle, rounded corners] {$Y_t$};
\node (phi) [below of=Y, draw, rectangle, rounded corners] {$\piphit$};

% Arrows
\draw[->] (X) edge[dashed] (Y);
\draw[->] (Y) -- (phi);
\draw[->] (Y) edge[loop above] (Y);
\draw[->] (phi) edge[loop below] (phi);
\draw[->] (phi) edge[bend left, color=red] (Y);
\draw[->] (phi) edge[dashed] (X);

% Labels
%\node [below of=X, node distance=1cm] {Latent \\Abstraction};
%\node [below of=Y, node distance=1cm] {Measurement Process};
\end{tikzpicture}
\caption{Interaction between Measurements $Y_t$, and Filtering process $\piphit$. Latent abstractions updates are \textit{implicitly} simulated (dashed line)}
\label{fig:interaction2}
\end{subfigure}
\end{figure}


==> packages-2.tex <==
% Acronyms
\usepackage{scalefnt,letltxmacro}
\LetLtxMacro{\oldtextsc}{\textsc}
\renewcommand{\textsc}[1]{\oldtextsc{\scalefont{1.10}#1}}
\usepackage[acronym,smallcaps,nowarn]{glossaries}
\glsdisablehyper
\makeglossaries
\usepackage{xspace}
\usepackage{float}
\usepackage{physics}
\usepackage[normalem]{ulem}

% Bullets
\usepackage{enumitem}

% Maths
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amsthm,thmtools}
\usepackage{booktabs}
% \usepackage[ruled,vlined]{algorithm2e}
\usepackage[]{microtype}

% Algorithms
% \usepackage[linesnumbered,ruled,vlined]{algorithm2e}
% \newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{gray}{#1}}
% \SetCommentSty{mycommfont}
% \SetKwInput{KwInput}{Input}
% \SetKwInput{KwOutput}{Output}

% hyperref

% cleverref
% \usepackage[capitalize,nameinlink,]{cleveref} %noabbrev
% \crefname{section}{\S}{\S\S}
% \Crefname{section}{\S}{\S\S}
% \creflabelformat{equation}{#2\textup{#1}#3}
% \providecommand\algorithmname{algorithm}

% color

\definecolor{shadecolor}{gray}{0.9}
\newcommand{\red}[1]{\textcolor{BrickRed}{#1}}
\newcommand{\orange}[1]{\textcolor{BurntOrange}{#1}}
\newcommand{\green}[1]{\textcolor{OliveGreen}{#1}}
\newcommand{\blue}[1]{\textcolor{MidnightBlue}{#1}}
\newcommand{\sky}[1]{\textcolor{SkyBlue}{#1}}
\newcommand{\gray}[1]{\textcolor{black!60}{#1}}
\definecolor{mylightgray}{gray}{0.94}

% counter for table
\makeatletter
\@ifundefined{c@rownum}{%
	\let\c@rownum\rownum
}{}
\@ifundefined{therownum}{%
	\def\therownum{\@arabic\rownum}%
}{}
\makeatother

% Other           
\DeclareRobustCommand{\parhead}[1]{\textbf{#1}~}

% For crossferencing across documents
\makeatletter
\newcommand*{\addFileDependency}[1]{% argument=file name and extension
	\typeout{(#1)}
	\@addtofilelist{#1}
	\IfFileExists{#1}{}{\typeout{No file #1.}}
}
\makeatother
\newcommand*{\myexternaldocument}[1]{%
	\externaldocument{#1}%
	\addFileDependency{#1.tex}%
	\addFileDependency{#1.aux}%
}
% % Figures
% \usepackage{nidanfloat}
% \usepackage[font=footnotesize,labelfont=bf,tableposition=top]{caption}
\usepackage{tikz}
\usepackage{graphicx}
% \usepackage[]{subcaption}   %% Already defined
% \usepackage{wrapfig}

\newcommand{\rulesep}{\unskip\ \hrule\ }

\usepackage{pgfplots}
\pgfplotsset{compat=1.6}
\usepgfplotslibrary{groupplots}
%% Use sans serif font for pictures
\tikzstyle{every picture}+=[font=\sffamily]
\tikzstyle{optimized} = [circle,fill=white,draw=black, dashed,inner sep=1pt, minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
\pgfkeys{/pgf/number format/.cd,1000 sep={}}
\pgfplotsset{
	tick label style = {font=\sffamily},
	every axis label/.append style={font=\sffamily},
	typeset ticklabels with strut,
}
\pgfplotsset{every axis/.append style={
			every x tick label/.append style={font=\fontsize{6pt}{6pt}\sffamily, yshift=.5ex,},
			every y tick label/.append style={font=\fontsize{6pt}{6pt}\sffamily, xshift=.5ex},
			every y label/.append style={xshift=10ex, font=\sffamily},
			every x label/.append style={yshift=3ex, font=\sffamily},
			every title/.append style={font=\sffamily}
		},
}
\pgfplotsset{
	xticklabel={$\mathsf{\pgfmathprintnumber{\tick}}$},
	yticklabel={$\mathsf{\pgfmathprintnumber{\tick}}$},
}
\pgfplotsset{every axis title/.append style={yshift=-1ex}}
\newlength\figureheight
\newlength\figurewidth
\usepgfplotslibrary{external}
\tikzexternalize[mode=list and make]
\tikzexternaldisable
\newcommand{\tikzfile}[1]{
	\tikzsetnextfilename{#1}%  
	\input{#1.tikz}
}
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
		\node[shape=circle,draw,inner sep=2pt] (char) {\tiny #1};}}


% ********************************************************************
% Notes and todos
% ********************************************************************
% \usepackage[colorinlistoftodos,
% 	% disable,
% 	textsize=scriptsize,
% 	linecolor=red!30,
% 	bordercolor=red!30,
% 	backgroundcolor=red!10]{todonotes}
% \makeatletter
% \renewcommand{\todo}[2][]{\tikzexternaldisable\@todo[#1]{#2}\tikzexternalenable}
% \makeatother
% \newcommand{\note}[1]{\todo[linecolor=BurntOrange,backgroundcolor=BurntOrange!25,bordercolor=BurntOrange, inline, ]{\color{BurntOrange!80!black}{\textbf{\textit{#1}}}}}


% \usepackage[most]{tcolorbox}
% \newenvironment{highlight}%
% {\begin{tcolorbox}[toprule=2mm,left=4pt,right=4pt,top=0pt,bottom=1pt,boxsep=2pt, before skip = 2ex, after skip =2ex]}{\end{tcolorbox}}
% \tcbset{boxsep=4pt,left=2pt,right=2pt,top=-0pt,bottom=0pt}


\newcommand\noteMF[1]{{\color{red}{\footnotesize {\textbf{\textsc{MF}}: ``#1''}\xspace}}}
\newcommand\noteSR[1]{{\color{blue}{\footnotesize {\textbf{\textsc{SR}}: \textit{``#1''}}\xspace}}}
\newcommand\notePM[1]{{\color{orange}{\footnotesize {\textbf{\textsc{PM}}: ``#1''}\xspace}}}
\newcommand\noteGF[1]{{\color{violet}{\footnotesize {\textbf{\textsc{GF}}: ``#1''}\xspace}}}
\newcommand\noteEB[1]{{\color{green}{\footnotesize {\textbf{\textsc{EB}}: ``#1''}\xspace}}}


\usepackage{url}

% \usepackage{xr}
% \externaldocument{supplementary}

%\usepackage{algorithm}
%\usepackage{algorithmic}
% \usepackage{subcaption}

\usepackage{tikz}
\usepackage{graphicx}
\usepackage{xcolor}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{bm}
\usepackage{amsthm} % theorems and proofs


% \declaretheorem[name=Theorem]{theorem}
% \declaretheorem[name=Lemma]{lemma}
% \declaretheorem[name=Proposition]{proposition}
% \declaretheorem[name=Corollary]{corollary}%numberwithin=section
% \declaretheorem[name=Definition]{definition}
% \declaretheorem[name=Condition]{condition}
% \declaretheorem[name=Assumption]{assumption}
% \declaretheorem[name=Example]{example}


%\newtheorem{theorem}{Theorem}
%\newtheorem{proposition}{Proposition}
%\newtheorem{lemma}{Lemma}
%\newtheorem{sublemma}{Lemma}[lemma]
%\newtheorem{corollary}{Corollary}
%\newtheorem{definition}{Definition}

\usepackage{adjustbox}
\usepackage{multirow}
\usepackage{mathtools}
%\DeclareMathOperator{\Hessian}{H}
%\DeclareMathOperator{\Hessian}{\mathbf{H}}
\DeclareMathOperator{\Hessian}{Hess}

\usepackage{xspace}

%\hypersetup{draft}
\newcommand{\redquestionmark}{\textbf{\textcolor{red!60!black}{?}}}




